Cache Subsidies for an Optimal Memory for Bandwidth Tradeoff in the Access Network

While the cost of the access network could be considerably reduced by the use of caching, this is not currently happening because content providers (CPs), who alone have the detailed demand data required for optimal content placement, have no natural incentive to use them to minimize access network operator (ANO) expenditure. We argue that ANOs should therefore provide such an incentive in the form of direct subsidies paid to the CPs in proportion to the realized savings. We apply coalition game theory to design the required subsidy framework and propose a distributed algorithm, based on Lagrangian decomposition, allowing ANOs and CPs to collectively realize the optimal memory for bandwidth tradeoff. The considered access network is a cache hierarchy with per-CP central office caches, accessed by all ANOs, at the apex, and per-ANO dedicated bandwidth and storage resources at the lower levels, including wireless base stations, that must be shared by multiple CPs.

==> abstract.tex <==
\begin{abstract}

It is widely recognized that caching at the edge of network  can contribute to significantly reduce the infrastructure  costs of access network operators (ANOs). However,  in practice, content is rarely cached  at any site closer to the users than points of presence (PoPs), due to the lack of incentives that  content provides (CPs) have to cooperate with ANOs.  We believe that network operators can generate such an incentive by financially rewarding those CPs,  which are willing to  cooperate with them. The gain stemming  by  optimal memory for bandwidth  tradeoffs  is potentially enough to ensure significant benefits  to  ANOs, CPs and ultimately end-users.
	
We propose a value sharing scheme where CPs maximize their subsidy by optimally placing content items in an access network cache hierarchy   rooted at the central office. We find out  how the cost of the CO cache and corresponding CP subsidy must be partitioned among  multiple ANOs.

Furthermore we design a distributed iterative algorithm  based on Lagrangian decomposition. CPs compute their optimal content placements in the cache hierarchy, given unit bandwidth and storage shadow prices, while ANOs fix shadow prices so to maximize utilization of limited resources. Neutrality is assured by our proposed scheme, indeed same prices are applied to all CPs, while content items are placed independently of the CP they belong to.	
\end{abstract}

%\begin{IEEEkeywords}
%Computer Society, IEEE, IEEEtran, journal, \LaTeX, paper, template.
%\end{IEEEkeywords}
